SpecSAR-Former: A Lightweight Transformer-based Network for Global LULC Mapping Using Integrated Sentinel-1 and Sentinel-2

Recent approaches in remote sensing have increasingly focused on multimodal data, driven by the growing availability of diverse earth observation datasets. Integrating complementary information from different modalities has shown substantial potential in enhancing semantic understanding. However, existing global multimodal datasets often lack the inclusion of Synthetic Aperture Radar (SAR) data, which excels at capturing texture and structural details. SAR, as a complementary perspective to other modalities, facilitates the utilization of spatial information for global land use and land cover (LULC). To address this gap, we introduce the Dynamic World+ dataset, expanding the current authoritative multispectral dataset, Dynamic World, with aligned SAR data. Additionally, to facilitate the combination of multispectral and SAR data, we propose a lightweight transformer architecture termed SpecSAR-Former. It incorporates two innovative modules, Dual Modal Enhancement Module (DMEM) and Mutual Modal Aggregation Module (MMAM), designed to exploit cross-information between the two modalities in a split-fusion manner. These modules enhance the model's ability to integrate spectral and spatial information, thereby improving the overall performance of global LULC semantic segmentation. Furthermore, we adopt an imbalanced parameter allocation strategy that assigns parameters to different modalities based on their importance and information density. Extensive experiments demonstrate that our network outperforms existing transformer and CNN-based models, achieving a mean Intersection over Union (mIoU) of 59.58%, an Overall Accuracy (OA) of 79.48%, and an F1 Score of 71.68% with only 26.70M parameters. The code will be available at https://github.com/Reagan1311/LULC_segmentation.

==> beifen.tex <==
% Ma et al. introduced FTransUNet \cite{ma2024multilevel}, a multilevel multimodal fusion scheme that combines CNNs and Vision Transformers (VIT) to enhance semantic segmentation of remote sensing data. The network extracts shallow-level features through convolutional layers and Shallow-Level Feature Fusion (SFF) modules, and employs advanced attention mechanisms to capture highly distinguishable cross-modal features, significantly improving segmentation accuracy. Gbodjo et al. \cite{gbodjo2021multisensor} developed a deep learning framework designed to integrate multimodal remote sensing data, primarily for multimodal analysis in downstream tasks such as land cover mapping. The paper designed a patch-based multi-branch CNN, which employs  Visual Geometry Group (VGG)-like \cite{simonyan2014very} encoders to handle their respective input signals. Additionally, the research introduced a self-distillation strategy that uses the final predictions from multisource data to guide the learning of encoders for each data source. Yu et al. \cite{yu2023deep} proposed a deep learning framework designed to segment urban functional zones by integrating remote sensing images with point-of-interest data. This framework uses a CNN to extract visual features from the remote sensing images and social features from the point-of-interest data. These features are then merged using a feature fusion module, effectively delineating urban functional zones.

